MOON, an Operational Modeling of the Medical Pathway

The use of digitized medical records is growing in importance. Unfortunately digitized medical records suffer from a lack of coordination between medical actors and medical departments, furthermore the proposed standards focus more on data than on medical practices themselves. In this context, reconstructing a patient's global medical history is virtually impossible. Even worse, the management of this global medical pathway falls to the patient, who lacks the necessary medical knowledge to handle it efficiently. We propose a new framework named MOON whose underlying concepts and structures allow for a specification of medical practices across virtually any medical field and then can describe any medical pathway involving the specified practices. This approach also enables the creation of comprehensive, patient-centered medical records that can be shared among all medical stakeholders. Adopting this type of framework would help improve the efficiency of care and, consequently, patient health.

==> Packages_and_macros.tex <==
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{tikz}
\usepackage{xargs}
\usepackage{ifthen}
\usepackage{amssymb}
\usepackage{xparse}
\usepackage{hyperref}
\usetikzlibrary{patterns}
\usetikzlibrary{math}
\usetikzlibrary{arrows.meta}
\usetikzlibrary{calc}
\usetikzlibrary{shapes.multipart}
\usetikzlibrary{shadows}
\usetikzlibrary{shadings}
\usepackage{cancel}
\usepackage{xstring}
\usepackage[gray]{xcolor}
\usepackage{soul}

%--------------------------------------------------------------
% Macros for schema specifications
%--------------------------------------------------------------
\input{general_macros}
\input{specs_macros}
\input{program_macros}

\sethlcolor{yellow!50!white}
\newcommand{\highlight}[1]{\textcolor{red!50!black}{\hl{#1}}}

\newcommand{\modifDC}[2]{{\color{lightgray} #1}\highlight{#2 (DC)}}
\newcommand{\remarkDC}[2]{\highlight{#1}\marginpar[right]{\tiny DC : #2}}

\newcommand{\modifJH}[2]{{\color{lightgray} #1}\highlight{#2 (JH)}}
\newcommand{\remarkJH}[2]{\highlight{#1}\marginpar[right]{\tiny JH : #2}}


